Optimal Oblivious Algorithms for Multi-way Joins

In cloud databases, cloud computation over sensitive data uploaded by clients inevitably causes concern about data security and privacy. Even when encryption primitives and trusted computing environments are integrated into query processing to safeguard the actual contents of the data, access patterns of algorithms can still leak private information about the data. Oblivious Random Access Memory (ORAM) and circuits are two generic approaches to address this issue, ensuring that access patterns of algorithms remain oblivious to the data. However, deploying these methods on insecure algorithms, particularly for multi-way join processing, is computationally expensive and inherently challenging. In this paper, we propose a novel sorting-based algorithm for multi-way join processing that operates without relying on ORAM simulations or other security assumptions. Our algorithm is a non-trivial, provably oblivious composition of basic primitives, with time complexity matching the insecure worst-case optimal join algorithm, up to a logarithmic factor. Furthermore, it is cache-agnostic, with cache complexity matching the insecure lower bound, also up to a logarithmic factor. This clean and straightforward approach has the potential to be extended to other security settings and implemented in practical database systems.

==> algorithm.tex <==
  As described in Algorithm~\ref{alg:framework}, our framework consists of the following three components:
   
   {\bf Pre-processing.} If there exists an optimal fractional edge covering $W^*(\cdot)$ such that $W^*(e) = 0$ or $W^*(e) = 1$ for some relation $e \in \E$, we can simplify the join query as follows:
   \begin{itemize}[leftmargin=*]
       \item {\bf Case 1: $W^*(e) = 0$.} We conceptually remove the relation $e$ from $\E$. But the optimality of $W^*$, the optimal fractional edge covering number of the residual join query $\Q' = (\V, \E - \{e\})$ is still $|W^*|$. Then, we invoke the whole algorithm recursively for computing $\Q'$ on the residual instance $\R' = \R - \{R_e\}$, whose join result is denoted as $\Q'(\R')$. At last, we just return the semi-join between $\Q'(\R')$ and $R_e$ as the final join results. 
       \item {\bf Case 2: $W^*(e) = 1$.} We conceptually remove all attributes in $e$ from $\V$. But the optimality of $W^*$, the optimal fractional edge covering number of the residual join query $\Q' = (\V -e , \E[\V-e])$ is $|W^*|-1$. Then, we invoke the whole algorithm recursively for computing $\Q'$ on the residual instance $\R'$ as defined in line 5, whose join result is denoted as $\Q'(\R')$. At last, we just compute the Cartesian product between $\Q'(\R')$ and $R_e$, and apply semi-joins by all relations $R_{e'}$ with $e' \cap e \neq \emptyset$. 
   \end{itemize}

    {\bf Decompose the join query.} Whenever there exists an arbitrary pair of attributes $x,y$ such that that there is no relation $e \in \E$ with $x,y \in e$, we can perform the following procedure to decompose the join query. More specifically, we consider two subqueries $\Q_{\bar{x}}$ and $\Q_{\bar{y}}$ that contain all attributes in $\V$ except $x$ and $y$ separately. Correspondingly, the residual instances derived for $\Q_{\bar{x}}$ and $\Q_{\bar{y}}$, denoted as $\R_{\bar{x}}$ and $\R_{\bar{y}}$ are the projections of relations onto $\V - \{x\}$ and $\V - \{y\}$ separately. We next invoke the whole algorithm recursively for computing the join results $\Q_{\bar{x}}(\R_{\bar{x}})$ and $\Q_{\bar{y}}(\R_{\bar{y}})$
     separately. 
     At last, we simply invoke the relaxed oblivious two-way join to compute $\Q_{\bar{x}}(\R_{\bar{x}}) \Join \Q_{\bar{y}}(\R_{\bar{y}})$ under the threshold of AGM bound. The correctness of this step lies in Lemma~\ref{lem:decompose}.

       \begin{algorithm}
       \caption{{\sc ObliviousJoin}$(\Q,\R)$}
        \label{alg:framework}
        \If{$\Q$ is disconnected}{
        $\Q_1,\Q_2,\cdots,\Q_k \gets$ connected sub-queries of $\Q$\;
        $\R_1,\R_2,\cdots, \R_k \gets$ sub-instances for $\Q_1,\Q_2,\cdots,\Q_k$\;
        \ForEach{$i \in [k]$}{
            $\S_i \gets \textsc{OblivousJoin}(\Q_i, \R_i)$\;
        }
        \Return $\textsc{NestedLoop}(\S_1(\V_1),\S_2(\V_2), \cdots,\S_k(\V_k))$\;
        }
        \ElseIf{$|\E|=1$, say $\E = \{e\}$}{
            \Return $R_e$\;
        }
        \ElseIf{$\exists$ an optimal fractional edge covering $W^*(\cdot)$ for $\Q$ such that $W^*(e) =0$ for some $e \in \E$}{
        $\mathcal{S} \gets \textsc{ObliviousJoin}((\V,\E-\{e\}),\R - \{R_e\},N)$\;
        \Return $\textsc{SemiJoin}(\mathcal{S}, R_e)$\;
        }
        \ElseIf{$\exists$ an optimal fractional edge covering $W^*(\cdot)$ for $\Q$ such that $W^*(e) =1$ for some $e \in \E$}{
        $\R' \gets \{\pi_{e' -e} R_{e'}: e' \cap e \neq \emptyset\} \cup \{R_{e'}: e' \cap e = \emptyset\}$\;
        $\mathcal{S} \gets \textsc{ObliviousJoin}((\V-e,\E[\V-e]), \R', N)$\;
        $\mathcal{S} \gets \textsc{NestedLoop}(\mathcal{S}, R_e)$\;
        \lForEach{$e' \in \E'$}{
            $\mathcal{S} \gets \textsc{SemiJoin}(\mathcal{S}, R_{e'}, N)$}
        \Return $\mathcal{S}$\;
        }
        \ElseIf{
        $\exists (x,y) \in \V \times \V$ such that  $x\neq \y$ and there exists no relation $e \in \E$ such that $x,y \in e$}{
        $\Q_{\bar{x}} \gets (\V-x, \E[\V-\{x\}])$\;
        $\R_{\bar{x}} \gets \left\{\pi_{e-x}R_e: e \in \E\right\}$\;
        $\Q_{\bar{y}} \gets (\V-y, \E[\V-\{y\}])$\;
        $\R_{\bar{y}} \gets \left\{\pi_{e-y}R_e: e \in \E\right\}$\;
        $\mathcal{S}_{\bar{x}} \gets \textsc{\sc ObliviousJoin}(\Q_{\bar{x}}, \R_{\bar{x}}, N)$\;
        $\mathcal{S}_{\bar{y}} \gets \textsc{\sc ObliviousJoin}(\Q_{\bar{y}}, \R_{\bar{y}}, N)$\;
        $W^* \gets $ an optimal fractional edge covering of $\Q$\;
        \Return $\textsc{RelaxedObliviousTwoJoin}(\mathcal{S}_1,\mathcal{S}_2, N^{|W^*|})$\;
        }
        \Else(\tcp*[h]{\color{blue}{$\Q$ must be a non-conformal clique}}){
        \Return $\textsc{ObliviousNCC}(\Q,\R, N)$\; 
        }
   \end{algorithm}


     \begin{lemma}
     \label{lem:decompose}
         $\Q_{\bar{x}}(\R_{\bar{x}}) \Join \Q_{\bar{y}}(\R_{\bar{y}}) = \Q(\R)$.
     \end{lemma}
     
    \noindent {\bf Reach the hard case.} When Algorithm~\ref{alg:framework} reaches line 19, the join query is denoted as a {\em non-conformal clique join}. We will tackle non-conformal clique join separately in Section~\ref{sec:non-conformal}. 
   
    \begin{definition}[Non-Conformal Join]
    \label{def:non-conformal}
       A join query $\Q=(\V,\E)$ is non-conformal if (\romannumeral 1) for every pair of attributes $x,y \in \V$, there exists a relation $e \in \E$ such that $x,y\in e$; and (\romannumeral 2) there exists no optimal fractional edge covering $W^*(\cdot)$ for $\Q$ such that $W^*(e) = 0$ or $W^*(e)=1$ for some relation $e \in \E$.
    \end{definition}

    \begin{lemma}
        In a non-conformal join $\Q = (\V,\E)$, %there exists no relation $e \in \E$ such that $e = \V$, and 
        $|\E| \le |\V|$.
    \end{lemma}

    % \zhiang{For this definition, we even have $|\mathcal{V}|?|\mathcal{E}|$??? Assume the $\mathcal{V}$ constraints are in the form of $x_v + \sum\limits_{v\in e} R_e=1$ for any  $v\in\mathcal{V}$. By the definition, for any optimal solution for the above LP on $|\mathcal{E}|+|\mathcal{V}|$ variables and $|\mathcal{V}|$ constraints, the number of non-zero entries of $W^*()$ is $|\mathcal{E}|$. The $\mathrm{rank}$ of constraints matrix is $|\mathcal{E}|$, otherwise, one $W^*(e)$ can be represented by the other $W^*(e')'s$.  Hence all the constraints are linearly independent?}

    \begin{proof}
    %If there exists a relation $e \in \E$ such that $e = \V$, there must exist an optimal fractional edge covering $W^*(\cdot)$ such that $W^*(e)=1$ and $W^*(e') =0$ for every remaining relation $e' \in \E - \{e\}$, coming to the contradiction of the definition of a non-conformal join query. 
    %
    Consider the polyhedron of the fractional edge covering defined on $|\E|$ variables and $|\V| + |\E|$ constraints. The extreme point corresponding to an arbitrary optimal fractional edge covering $W^*(\cdot)$ must be the intersection of exactly $|\E|$ (linearly independent) tight constraints. Note that $W^*(e) > 0$ holds for every relation $e \in \E$. Then, $|\E|$ constraints out of the remaining $|\V|$ constraints in terms of $\sum_{e: x \in e} W^*(e) \ge 0$ must be tight, i.e., $|\E| \le |V|$.
    \end{proof}

    At last, we show that the recursion finishes in $O(1)$ iterations. Moreover, the size of the join query (in terms of the number of attributes and relations) keep decreases, until it reaches the base case that $|\E|=1$, or it falls into a non-conformal clique.

     \begin{example}
       \label{ex:three}
       Consider an example join query $\Q = R_1(x_1,x_2,x_3) \\ \Join R_2(x_1,x_5,x_6) \Join R_3(x_2,x_4,x_5) \Join R_4(x_3,x_4,x_6)$ with the optimal fractional edge covering number as $2$. We first identify a pair of attributes $x_1,x_4$ that do not appear in any common relation, which yields two subqueries $\Q_1 = R_1(x_1,x_2,x_3) \Join R_2(x_1,x_5,x_6) \Join R_3(x_2,x_5) \Join R_4(x_3,x_6)$ and $\Q_2 = R_1(x_2,x_3) \Join R_2(x_5,x_6) \Join R_3(x_2,x_4, x_5) \Join R_4(x_3,x_4, x_6)$.

       
       For $\Q_1$, we further identify a pair of attributes $x_2,x_6$ that do not appear in any common relation, which yields another two subqueries
       $\Q_{11} = R_1(x_1,x_2,x_3) \Join R_2(x_1,x_5) \Join R_3(x_2,x_5) \Join R_4(x_3)$ and $\Q_{12} = R_1(x_1,x_3) \Join R_2(x_1,x_5,x_6) \Join R_3(x_5) \Join R_4(x_3,x_6)$. As both $\Q_{11}$ and $\Q_{12}$ have an optimal fractional edge covering that is also integral, then they can be computed within $O(N^2)$ time.
       
       For $\Q_2$, we further identify 
       a pair of attributes $x_2,x_6$ that do not appear in any common relation, which yields another two subqueries
       $\Q_{21} = R_1(x_2,x_3) \Join R_2(x_5) \Join R_3(x_2,x_4, x_5) \Join R_4(x_3,x_4)$ and $\Q_{22} = R_1(x_3) \Join R_2(x_5,x_6) \Join R_3(x_4, x_5) \Join R_4(x_3,x_4,x_6)$. Similarly, as both $\Q_{21}$ and $\Q_{22}$ have an optimal fractional edge covering that is also integral, then they can be computed within $O(N^2)$ time.   
   \end{example}

   %\begin{example}
   %    Consider the $(k,\ell)$-uniform join query, where every subset of $\ell$ attributes from all $k$ attributes corresponds to a relation. For example, $(d,d-1)$-uniform join is a Loomis-Whitney join. Suppose $k = 6$ and $\ell=3$. Suppose $\V = \{A,B,C,D,E,F\}$. There exists an optimal fractional edge covering $W^*(\cdot)$ such that $W^*(e) = \frac{1}{2}$ for every relation $e \in \{\texttt{ABD}, \texttt{BCE}, \texttt{ACF}, \texttt{DEF}\}$, and $W^*(e') = 0$ for every remaining relation $e'$. 
   %    
   %    Consider the residual join query $\Q = R_1(ABD) \Join R_2(BCE) \Join R_3(ACF) \Join R_4(DEF)$. We first identify a pair of attributes $A, E$ that do not appear in any common relation, which yields two sub-queries $\Q_1 = R_1(ABD) \Join R_2(BC) \Join R_3(ACF) \Join R_4(DF)$ and $\Q_2 = R_1(BD) \Join R_2(BCE) \Join R_3(CF) \Join R_4(DEF)$. 
    %
    %   For $\Q_1$, we identify a pair of attributes $B,F$ that do not appear in any common relation, which yields two sub-queries $\Q_{11} = R_1(ABD) \Join R_2(BC) \Join R_3(AC) \Join R_4(D)$ and $\Q_{12} = R_1(AD) \Join R_2(C) \Join R_3(CF) \Join R_4(DF)$. As both $\Q_{11}$ and $\Q_{12}$ have an optimal fractional edge covering that is also integral, they can be computed in $O(N^2)$ time.
    %
    %   For $\Q_2$, we identify a pair of attributes $B, F$ that do not appear in any common relation, which yields two sub-queries $\Q_{21} = R_1(BD) \Join R_2(BCE) \Join R_3(C) \Join R_4(DE)$ and $\Q_{22} = R_1(D) \Join R_2(CE) \Join R_3(CF) \Join R_4(DEF)$. As both $\Q_{21}$ and $\Q_{22}$ have an optimal fractional edge covering that is also integral, they can be computed in $O(N^2)$ time.


   %\end{example}

    %\zhiang{
     %\begin{example}
    %   Consider an example join query $Q=R_1(A,B,C)\Join R_2(A,B,E,F) \Join R_3(A,D,G) \Join R_4(B,D,G) \Join R_5(C,D,F)\Join R_6(C,E,G)$ with the optimal fractional edge covering number as $\frac{15}{7}$. One optimal fractional edge covering is $W^*(Q)=(\frac{1}{7},\frac{4}{7},\frac{2}{7},\frac{2}{7}, \frac{3}{7},\frac{3}{7})$. Since the constraint matrix of covering LP has rank $6$, $W^*(Q)$ is unique. For optimal fractional vertex packing, we have infinite optimal solutions and two of them are $\tau^*_1(Q)=(\frac{2}{7},\frac{2}{7}, \frac{3}{7}, \frac{1}{7},\frac{0}{7},\frac{3}{7}, \frac{4}{7})$ and $\tau^*_2(Q) =(\frac{2}{7},\frac{2}{7}, \frac{3}{7}, \frac{2.5}{7},\frac{1.5}{7},\frac{1.5}{7}, \frac{2.5}{7})$. (Can we have two zero entries in $\tau^*(Q)$? We can assume that $\tau^*_G$ is linearly represented by $\tau^*_A,\cdots,\tau^*_F$ since the rank is 6?) 
    
        %This is not a non-conformal clique.
        %Note that attributes $D$ and $E$ do not appear in any relation simultaneously, which yields two subqueries $\Q_1=R_1(A,B,C)\Join R_2(A,B,F) \Join R_3(A,D,G) \Join R_4(B,D,G) \Join R_5(C,D,F)\Join R_6(C,G)$ and $\Q_2=R_1(A,B,C)\Join R_2(A,B,E,F) \Join R_3(A,G) \Join R_4(B,G) \Join R_5(C,F)\Join R_6(C,E,G)$.
        %For $\Q_1$, we further identify a pair of attributes $F,G$ that do not appear in any common relation, which yields two subqueries \[\Q_{11} =R_1(A,B,C)\Join R_2(A,B,F) \Join R_3(A,D) \Join R_4(B,D) \Join R_5(C,D,F)\] $\tau^*= ({2\over5},{2 \over 5}, {1 \over 5}, {3 \over 5}, {1 \over 5})$ and $\rho^* = ({2\over5},{2 \over 5}, {1 \over 5}, {1 \over 5}, {3 \over 5})$. \[\Q_{12}=R_1(A,B,C)\Join R_2(A,B) \Join R_3(A,D,G) \Join R_4(B,D,G) \Join R_5(C,D)\Join R_6(C,G)\] Note that $\Q_{11}$ and $\Q_{12}$ are non-conformal cliques.
   %\end{example}
   %}
   
   
    \section{Non-Conformal Clique Joins}
   \label{sec:non-conformal}


   %\begin{figure}
   %    \centering
   %    \includegraphics[scale=0.9]{img/example.pdf}
   %    \caption{An illustration of Algorithm~\ref{alg:framework} on Example~\ref{ex:three}.}.
   %    \label{fig:exmample}
   %\end{figure}

   \begin{example}[Odd-length Cycle Join]
   \label{ex:odd-length-cycle}
      A odd-length cycle join $\Q = (\V,\E)$ is defined with $\V= \{x_1, x_2, \cdots, x_n\}$ and $\E = \{e_i = \{x_i, x_{(i+1) \mod n}\}: i \in [n]\}$. We proceed with an edge $e_1 = (x_1,x_2)$. If $n=3$, this is exactly the triangle join, which has been resolved. We next focus on $n \ge 5$. We start with an arbitrary pair of attributes that do not appear together in some relation, say $(x_1,x_3)$, and get two sub-queries $\Q[\V- \{x_1\}],\Q[\V- \{x_3\}]$. As $\Q[\V- \{x_1\}]$ is acyclic, it admits an optimal fractional edge covering that is also integral. Hence, it can be computed within $O\left(N^{n/2}\right)$ time. The similar argument applies for $\Q[\V- \{x_3\}]$. The remaining two-way join can be computed within $O(N^{n/2})$ time. 
   \end{example}

   \begin{example}[Binary-relation Join]
   \label{ex:binary-relation}
       A join query $\Q= (\V,\E)$ is binary if $|e|\le 2$ holds for every $e \in \E$. It has been proved by~\cite{} that there exists an optimal fractional edge covering $W^*$ of any binary-relation join query $\Q$ that (1) $W^*(e) \in \{0,\frac{1}{2},1\}$; (2) the collection of edges $e$ for which $W^*(e) = 1$ form a set of vertex-disjoint stars $S$; (3) the collection of edges $e$ for which $W^*(e) = \frac{1}{2}$ form a set of vertex-disjoint odd-length cycles $C$, which are also vertex-disjoint from $S$. By plugging this nice property into Algorithm~\ref{alg:general}, it suffices to compute the join results for each odd-length cycle, then compute the Cartesian product of all edges $e$ with $W^*(e) =1$ together with all materialized cycles, and finally filter by all edges $e$ with $W^*(e) =0$.
   \end{example}

   

==> intro.tex <==
\section{Introduction}

\subsection{Problem Definition}
\label{sec:preliminary}

\paragraph{Multi-way Join.} A (natural) join query can be represented as a triple $\Q = (\V,\E)$~\cite{abiteboul1995foundations}, where $\V$ is the set of attributes, and $\E \subseteq 2^{\V}$ is the set of  relations. Let $\dom(x)$ be the domain of attribute $x$. An instance of $\Q$ is a function $\R$ that maps each $e \in \E$ into a set of tuples $R_e$, where each tuple $t \in R_e$ specifies a value in $\dom(v)$ for each attribute $v \in e$. The join results of $\Q$ over instance $\mathcal{R}$, denoted by $\Q(\R)$, is the set of all combinations of tuples, one from each $R_e$, that share common values for their common attributes, i.e., 
\begin{equation}
\label{eq:QR}
    \Q(\R) = \{t \in \prod_{x \in \V} \dom(x) \mid \forall e \in \E, \exists t_e \in R_e, \pi_{e} t = t_e\}.
\end{equation} 

Let $N = \sum_{i \in [m]} |R_e|$ be the {\em input size} of instance $\R$, i.e., the total number of tuples over all relations. Let $\OUT = |\Q(R)|$ be the {\em output size} of join query $\Q$ over instance $\R$. We study the data complexity~\cite{abiteboul1995foundations} of
join algorithms by measuring their running time in terms of input and output size of instance. We assume the size of $\Q$, such as $|\V|$ and $|\E|$, to be bounded by a constant.


For a join query $\Q = (\V,\E)$ and a subset of attributes $S \subseteq \V$, we denote the subquery restricted to attributes in $S$ as $\Q[S] = (\V,\E[S])$, where
     \[\E[S] = \{e \cap S: e \in \E\}\]
% It has been formally stated that $\max_{\R \in \mathbb{R}(N)}|\Q(\R)| \le \min_{\rho} \prod_{e \in \E} N^{\rho(e)}_e$where $\rho$ is a fractional edge cover of the hypergraph $(\V,\E)$.


%An important class of join queries is known as {\em acyclic join}~\cite{beeri1983desirability}. A multi-way join is acyclic if there exists a tree structure $\mathcal{T}$ of $\Q$ such that (1) there is a one-to-one correspondence between relations in $\Q$ and nodes in $\mathcal{T}$; (2) for every attribute $x \in \x$, the set of nodes containing $x$ form a connected subtree of $\mathcal{T}$.


\paragraph{Trusted and Untrusted Memory.} We adopt the model used by~\cite{arasu2013oblivious}. The query execution is performed within a {\em trusted memory} that cannot be accessed by adversaries. Input database and possibly intermediate results generated are stored (encrypted) in an {\em untrusted memory}, that can be accessed by adversaries. In particular, adversaries can observe the sequence of memory locations accessed and (encrypted) data
read/written, but they do not interfere with the query execution. In this paper, we consider $O(1)$ trusted memory.

\paragraph{Full Obliviousness.} The notion of obliviousness is defined with respect to memory accesses to the untrusted memory. We note that any memory access to the trusted memory is invisible to the adversary and do not affect security.
Let $\A$ be an algorithm, $\R$ be an arbitrary input instance to algorithm $\A$. 
We denote $\mathsf{Access}_\A(\R)$ as the sequence of memory addresses and each access is a read or write operator executed by $\mathcal{A}$ on instance $\R$. Moreover, $\mathsf{Access}_\A(\R)$ is also known as the ``access pattern'' of algorithm $\A$ on instance $\R$.

\begin{definition}[Full Obliviousness (FO)~\cite{goldreich1987towards, goldreich1996software}] 
\label{def:FO}
     An algorithm~$\mathcal{A}$ is fully oblivious if for any pair of instances $\R,\R'$ of input size $N$, $\mathsf{Access}_\A(\R)  \overset{\mathrm{\delta}}{\equiv} \mathsf{Access}_\A(\R')$, where $\delta$ is a negligible function in terms of $N$, i.e., $\delta < \frac{1}{N^c}$ for some constant $c$, and $\overset{\mathrm{\delta}}{\equiv}$ denotes that two distributions have statistical distance at most $\delta$.
\end{definition}

Intuitively, a fully oblivious algorithm displays almost identical access pattern on all instances with the same input size. 

\subsection{Review of Existing Results}

\paragraph{ORAM.}

\noindent{\bf Insecure Join Algorithms.} The classical Yannakakis algorithm~\cite{yannakakis1981algorithms} can compute an {\em acyclic join}\footnote{A join query $\Q$ is acyclic if there exists a tree structure $\mathcal{T}$ of $\Q$ such that (1) there is a one-to-one correspondence between relations in $\Q$ and nodes in $\mathcal{T}$; (2) for every attribute $x \in \x$, the set of nodes containing $x$ form a connected subtree of $\mathcal{T}$. See an example in Appendix~\ref{appendix:intro}.}\cite{beeri1983desirability, fagin1983degrees} with $O(N + \OUT)$ time. This is already instance-optimal, since any algorithm needs to read the input data and output every join result. Moreover, the PANDA algorithm can compute a general join with $O((N^w + \OUT)\cdot \polylog)$ time~\cite{abo2016faq}, where $w$ is the sub-modular width of the join query. In addition, worst-case optimal join algorithms~\cite{ngo2018worst} can compute a general join in $O(N^\rho)$ time, where $\rho$ is the fractional edge covering number of the join query (defined in Section~\ref{sec:preliminary}).

However, these algorithms are not fully oblivious. Output-sensitive algorithms have its total number of memory accesses depending on the output size, which can vary from a constant to a polynomially large number over instances with the same input size. To remedy this issue, one can resort to {\em worst-case padding} to remedy such a leakage, i.e., pad dummy access up to the worst case. But, this does not necessarily give us fully oblivious algorithms. The specific sequence of memory addresses can differ dramatically over instances with the same input size. We give an example of triangle join processing in Section~\ref{sec:preliminary} to show why worst-case optimal algorithm is not fully oblivious. 


%\begin{definition}[Acyclic Join~\cite{beeri1983desirability, fagin1983degrees}]
%
%\end{definition}

%\begin{figure}
%\includegraphics[scale=1.1]{img/join-tree-acyclic.pdf}
%    \centering
%    \caption{An example of join tree for acyclic join $\Q = R_1(x_1,x_2,x_3) \Join R_2(x_2, x_4) \Join R_3(x_2, x_3, x_5) \Join R_4(x_5, x_6) \Join R_5(x_3, x_7)$. It can be easily observed that every node corresponds to a distinct relation, and for every attribute, the set of nodes containing it form a connected subtree. As will be used in Section~\ref{sec:relaxed}, the join query $\Q$ with a subset attributes $\bar{\y} = \{x_1,x_2, x_3\}$ (in red) is free-connex, since adding another node containing all attributes in $\bar{\y}$ (i.e., another copy of $R_1$) to $\Q$ still results in an acyclic join. As will be used in Section~\ref{sec:WO-ORAM}, it is also a {\em free-connex join tree} of $(\Q, \bar{\y})$, such that for any $x \in \bar{\y}, x' \notin \bar{\y}$, $\textsf{top}(x')$ is not an ancestor of $\textsf{top}(x)$, where $\textsf{top}(\cdot)$ denotes the highest node that $x$ appears.}
%    \label{fig:acyclic}
%\end{figure}

\paragraph{Fully Oblivious Join Algorithms.} We note that only a few fully oblivious join algorithm have been designed in the literature. The naive nested-loop join algorithm is already fully oblivious, by computing the Cartesian product of input relations, but its time complexity is as large as $O(N^m)$, where $m$ is number of relations. Wang et al.~\cite{wang2022query} designed circuits for conjunctive queries (which captures joins as a special case), whose complexity matches the polymatroid bound up to poly-logarithmic factors. Running such a circuit will automatically yields a fully oblivious algorithm for an arbitrary join with $O(N^{\rho} \cdot \textsf{poly}\log N)$ time complexity. Meanwhile, incorporating the insecure worst-case optimal algorithm into the ORAM framework can yield a fully oblivious algorithm with the same time complexity asymptotically.

\paragraph{Relaxed Fully Oblivious Joins.} People have also investigated other relaxed notions of full obliviousness in join processing. One line of work considered releasing both input and output size in the join processing. Note that incorporating the insecure output-sensitive join algorithm into ORAM framework yields such a relaxed oblivious algorithm with $O((N^w+\OUT) \cdot \polylog N)$ time complexity.  Arasu et al.~\cite{arasu2013oblivious} studied a relaxed oblivious algorithm for acyclic joins running in $O((N+\OUT) \cdot \log N)$ time, without any dependency on the ORAM framework. However, these join algorithms are not fully oblivious, since neighboring databases can have dramatically different output sizes, which can be distinguished by counting the total number of memory accesses. An alternative of thwarting output size leakage, is to ask user to specify an upper bound on the output size, which could be too high, then there would be many wasted operations, or too small, then the algorithm even cannot finish correctly. If simply specifying a upper bound $N^\rho$ for $\OUT$, Arasu's algorithm becomes fully oblivious and also improves previous algorithms by polylog factors. Another line of work considered differentially oblivious algorithms, which are only required to display ``similar'' access patterns over ``neighboring'' instances that are close to each other, but only the simplest two-way join has been studied~\cite{chu2021differentially}. As differentially oblivious algorithm are not fully oblivious, we won't go into this direction further. 

%\paragraph{AGM bound.} The AGM bound~\cite{atserias2008size} is an upper bound on the output size of a join query $\Q$, which states that $|\Q(\I)| \le N^{\sum_{i \in [m]} \rho(i)}$ for an arbitrary function $\rho: [m] \to [0,1]$ such that $\sum_{i \in [m]: x \in \x_i} \rho(i) \ge 1$ for every $x \in \x$. We denote $N^{\rho^*}$ where $\rho^* = \min_\rho \sum_{i \in [m]} \rho(i)$ as the (tight) AGM bound, which is also simplified as $\AGM(\Q,N)$.



==> primitive.tex <==

%For join query $\Q = (\V,\E)$, a function $M: \V \to [0,1]$ is a fractional vertex packing if $\sum_{x \in e} M(x) \le 1$ for any relation $e \in \E$. The optimal fractional vertex packing is the one that maximizes the quantity $\sum_{x \in \V} M(x)$, captured by the following linear program: 
%\begin{align}
%\label{eq:vertex-pack}
%\textcolor{black}{\max} \ \sum_{v \in \V} M(v) \ \ \
%    \textrm{s.t. } \ \sum_{v: v \in e} M(v) & \le \log_2 N(e), \forall \textcolor{black}{e \in \E} \ \ \ \ \ \ \ \\
%    M(v) & \ge 0, \forall v \in \V \nonumber
%\end{align}
%The optimal value of (\ref{eq:vertex-pack}) is defined as the {\em fractional vertex packing number} of $\Q$, denoted as $\eta^*$.
%
%Note that (\ref{eq:vertex-pack}) is the dual of (\ref{eq:edge-cover}). Assume $W^*,M^*$ are the optimal fractional edge covering and packing of $\Q$. 
%The strong duality and complementary slackness properties imply the following properties:
%\begin{lemma}
%\label{lem:stong-duality}
%    $\sum_{e \in \E} W^*(e) = \sum_{v \in \V} M^*(x)$.
%\end{lemma}
%\begin{lemma}
%\label{lem:slackness}
%    If $W^*(e) > 0$, then $\sum_{x: x \in e} M^*(x) = 1$. 
%\end{lemma}

==> relaxed.tex <==
\section{Relaxed Oblivious Two-way Join}

Lastly, we complete our framework by presenting a relaxed binary join algorithm.
This relaxed binary join will take as input two relations $R_1, R_2$ and a public parameter $\tau \ge |R_1 \Join R_2|$, and output a table of $\tau$ elements contains all join results of $R_1 \Join R_2$. The access pattern of this algorithm does not reveal the information of input data, except the value of $\tau$. Arasu et al. \cite{arasu2013oblivious} first proposed an relaxed oblivious join algorithm but it requires $O(\log N)$ trusted memory, and involves rather complicated primitive without giving complete details~\cite{chang2021efficient}. We clean their algorithm with a simpler version, and reduce the size of trusted memory from $O(\log N)$ to $O(1)$.

%\begin{theorem}
%\label{the:relaxed-binary}
%    For any acyclic join, an instance $\R$ of input size $N$ and a parameter $\tau \ge |\Q(\R)|$, there is an algorithm that
%    can compute $\Q(\R)$ in $O((N + \tau) \cdot \log N)$ time using $O(1)$ trusted memory, whose access pattern only depends on $N$ and $\tau$.
%\end{theorem} 

The high-level idea is to simulate the sort-merge join algorithm without revealing the movement of pointers in the merge phase. Let $S = R_1(x_1,x_2) \Join R_2(x_2,x_3)$ be the join results sorted by $x_2,x_3,x_1$ lexicographically. The idea is to transform $R_1, R_2$ into a sub-relation of $S$ by keeping attributes $(x_1, x_2), (x_2,x_3)$ separately, without removing duplicates. Then, it suffices to do a one-to-one merge for obtaining the final join results. As described in Algorithm~\ref{alg:DO-join}, we construct these two sub-relations from the input relations $R_1,R_2$ via the following steps: (A running example is given in Figure~\ref{fig:binary}) 
 \begin{itemize}[leftmargin=*]
     \item {\bf (line 1)} count the number of tuples that each join value appear in each relation;
     \item {\bf (line 2-3)} attach each tuple with the number of tuples it can be joined in the other relation;
     \item {\bf (line 4)} expand each tuple to the annotated number of copies;
     \item {\bf (line 5-7)} prepare the expanded $R_1$ and $R_2$ with the correct ordering, as it appears in the final sort-merge join results;
      \item {\bf (line 8-9)} perform a one-to-one merge.
 \end{itemize}
 One missing primitive is \textsc{Expand}, which is the most technical part of Algorithm~\ref{alg:DO-join}, as well as the main separation from Arasu's algorithm. 
 In the remaining, we will focus on this critical primitive. 
 
 \begin{algorithm}[t]
 \caption{{\sc RelaxedTwoWay}$(R_1 \Join R_2, \tau)$}
 \label{alg:DO-join}
 \KwIn{Two relations $R_1(x_1,x_2),R_2(x_2,x_3)$ and a parameter $\tau \ge |R_1 \Join R_2|$;}
 \KwOut{A set of $\tau$ tuples containing join results of $R_1 \Join R_2$;}
 \textsc{Sort} $R_1$ by $(x_2,x_1)$ and $R_2$ by $(x_2,x_3)$ lexicographically\;
 \ForEach{$i \in \{1,2\}$}{$L_i \gets \textsc{CountByKey}(R_i, x_2)$\;}
 \textsc{Annotate} $R_{1}$ by $L_2$ and $R_{2}$ by $L_1$\;
 \lForEach{$i \in \{1,2\}$}{$\Tilde{R}_i \gets \textsc{Expand}(R_i, \tau)$}
 $\textsc{MultiNumber}(\Tilde{R}_2, \{x_2,x_3\})$\;
 \textsc{Sort} $\Tilde{R}_2$ by $(x_2, \textsf{num})$ lexicographically\;
 \ForEach{$j \in [\tau]$}{
    \wt $(t_j, t'_j)$ for the $j$-th tuple in $\Tilde{R}_1$ and $\Tilde{R}_2$ respectively\;
 }
 \end{algorithm}
 
 \begin{algorithm}[t]
 \caption{{\sc Expand}($R, \tau$)}
 \label{alg:FO-expand}
 \KwIn{A sequence $R =\langle (t_i, w_i):i\in[k]\rangle$ with $\tau \ge \sum_{i=1}^k w_i$;}
 \KwOut{A table $\Tilde{R}$ consisting of $w_i$ copies of $t_i$ for every $i \in [k]$, and is sorted by $t_i$;}
 $\mathsf{pos} \gets 1$, $X \gets \emptyset$\;
 \ForEach{$(t_i,w_i) \in R$}{\re $(t_i,w_i)$\; 
    \lIf{$w_i = 0$}{\wt $(\perp, +\infty)$ to $X$}
    \Else{\wt $(t_i, \mathsf{pos})$ to $X$\;
    $\mathsf{pos} \gets \mathsf{pos} + w_i$\;
    }
 } 
 $\mathsf{pos} \gets 1.5$\;
 \ForEach{$i \in [\tau]$}{
 \wt $(\perp, \mathsf{pos})$ to $X$\;
 $\mathsf{pos} \gets  \mathsf{pos}+1$\;
 }
 \textsc{Sort} $X$ by $\mathsf{pos}$ and break ties by putting $\perp$ after real tuples\;
 $t \gets \perp$\;
 \ForEach{$(\val,\mathsf{pos}) \in X$}{
    \re $(\val,\mathsf{pos})$\;
    \lIf{$\mathsf{pos} = +\infty$}{\wt $\perp$ to $\Tilde{R}$}
    \lElseIf{$\val \neq \perp$}{
        $t \gets \val$ \textbf{ and } \wt $\perp$ to $\Tilde{R}$}
    \lElse{\wt $t$ to $\Tilde{R}$}
 }
 \textsc{Compact} $\Tilde{R}$ and truncate it with the first $\tau$ elements\;
 \Return $\Tilde{R}$\;
 \end{algorithm}
 
 \paragraph{\textsc{Expand}.} Given a sequence of $\langle (t_i,w_i): w_i \in \mathbb{Z}^+, i \in [\ell]\rangle$, the goal is to expand each tuple $t_i$ with $w_i$ copies. The naive way of reading a pair $(t_i,w_i)$ and then writing $w_i$ copies does not preserve obliviousness, since the number of consecutive writes can leak the information. Alternatively, one might consider writing a fixed number of tuples after reading each pair, but the ordering of reading pairs is critical for avoiding dummy writes and avoiding too many pairs stored in trusted memory (this strategy is exactly adopted by \cite{arasu2013oblivious}). We present a much simpler algorithm by combining the full oblivious primitives. Suppose $\Tilde{R}$ is the output table of $R$, such that $\Tilde{R}$ contains $w_i$ copies of $t_i$, and any tuple $t_i$ comes before $t_j$ if $i < j$. As described in Algorithm~\ref{alg:FO-expand}, it consists of four phases:
 \begin{itemize}[leftmargin=*]
    \item {\bf (Line 1-7).} For each pair $(t_i, w_i) \in R$ with $w_i \neq 0$, we attach the beginning position of $t_i$ in $\Tilde{R}$, which is exactly $\sum_{j < i} w_j$. For the remaining pairs with $w_i = 0$, we note that these tuples won't participate in any join result. So, we replace them with $\perp$ and attach with the infinite position;
    \item {\bf (Line 8-11).} We pad $\tau$ dummy tuples, and attach them with consecutive numbers in $\{1,2,\cdots, \tau\} + 0.5$;
    \item {\bf (Line 12).} After sorting the well-defined positions, each tuple $t_i$ will be followed by $w_i$ dummy tuples, and all dummy tuples with infinite positions are put at last; 
    \item {\bf (line 13-19).} For each tuple $t_i$, we replace it with $\perp$ but the following $w_i$ dummy tuples with $t_i$.  After moving all dummy tuples to the last, the first $\tau$ elements are the desired output.
 \end{itemize}

 It can be easily checked that only the value of $k$ and $\tau$ are revealed from Algorithm~\ref{alg:FO-expand}.  But, when the procedure {\sc Expand} is invoked by Algorithm~\ref{alg:DO-join}, the value of $k$ exactly equals $N$, i.e., the size of input relations, so such a leakage does not cause any issue at all.

 \begin{theorem}
 \label{the:relaxed-binary}
    For $R_1(x_1, x_2) \Join R_2(x_2, x_3)$ of input size $N$ and a parameter $\tau \ge |R_1 \Join R_2|$, there is an algorithm that
    can compute $R_1 \Join R_2$ in $O((N + \tau) \cdot \log N)$ time using $O(1)$ trusted memory, whose access pattern only depends on $N$ and $\tau$.
 \end{theorem}

  \begin{figure*}
     \centering
     \includegraphics[scale=1.3]{img/two-table.pdf}
     \caption{A running example of Algorithm~\ref{alg:DO-join}.}
     \label{fig:binary}
 \end{figure*}
 
% We note that this primitive can also be used to build full oblivious algorithm for acyclic joins. More specifically, we can first replace all dangling tuples as $\perp$ using \semi, and then plugging the relaxed binary join into the pairwise framework. To obtain fully oblivious acyclic join algorithm, we can simply set the size threshold $\tau$ as $N^{\rho}$. 

%\newpage
%Consider an arbitrary instance $\R$ for $\pi_{A_1,A_2,\cdots,A_k} R_1(A,B) \Join R_2(A_2,B) \Join \cdots \Join R_k(A_k,B)$. We aim to show that if $\R$ has input size $N$ and output size $\OUT$, then $|R_1 \Join R_2 \Join \cdots \Join R_k| \le N \cdot \OUT^{1-\frac{1}{k}}$.
%
%We first compute for each value $b \in \dom(B)$, its {\em degree} $d_i(b)$ in relation $R_i$ for each $i \in [k]$, which is defined as the number of tuples displaying value $b$ in attribute $B$, i.e., $d_i(b) = |\sigma_{B=b} R_i|$. Let $\lambda_b = \prod_{i=1}^k d_{i}(b)$. It is not hard to see:
%	\begin{lemma}
%		\label{lem:star-out}
%		For any value $b \in \dom(B)$, $\lambda_b \le \OUT$. 
%	\end{lemma}
%
%For each value $b \in \dom(B)$, we define a permutation $\phi_b: [k] \to [k]$ such that $d_{\phi_b(i)}(b) \ge d_{\phi_b(j)}(b)$ for any $1 \le i \le j \le k$. Note that we can determine $\phi_b$ for all $b$'s by sorting all values in $d_i(b)$, breaking ties. There are {at most} $k!$ number of permutations in total. Each permutation $\phi$ over $[k]$ defines a subset of values in $\dom(B)$ as $B_\phi = \{b \in \dom(B): \phi_{b} = \phi\}$. 
%
%Consider an arbitrary permutation $\phi$. For each value $b \in B_\phi$,  we can show that \[\lambda_b = \prod_{j \in [k]} d_{\phi(j)}(b) \le d_{\phi(1)}(b) \cdot \lambda^{1-\frac{1}{k}}_b \le d_{\phi(1)}(b) \cdot \OUT^{1-\frac{1}{k}}\]
%Then, summing over all values in $B_\phi$, we get  \[\sum_{b \in B_\phi} \lambda_b \le \sum_{b \in B_\phi} d_{\phi(1)}(b) \cdot \OUT^{1-\frac{1}{k}} \le N \cdot \OUT^{1-\frac{1}{k}}\]
%Summing over all permutations, we get \[\sum_{\phi} \sum_{b \in B_\phi} \lambda_b = O\left(N \cdot \OUT^{1-\frac{1}{k}}\right)\]

==> triangle.tex <==

%We follow the similar idea of Algorithm~\ref{alg:triangle}, but with different execution plan. Each value $a \in \dom(x_1)$ is identified as {\em heavy} if its degree is greater than $\sqrt{N}$ in $R_1$ or $R_3$, and {\em light} otherwise. %Furthermore, each tuple in $R_1$ or $R_3$ is identified as {\em heavy} if its value on attribute $x_1$ is heavy, and {\em light} otherwise. We denote $R^H_i, R^L_i$ as the set of heavy and light tuples in $R_i$ for $i \in \{1,3\}$. %5For full obliviousness, we retrieve $R^H_1, R^L_1, R^H_3, R^L_3$ and pad dummy tuples to $N$ for each sub-relation. 

%We further partition light values in attribute $x_2$ into multiple disjoint groups such that the total degree of each group in $R_2$ or $R_3$ falls in $(\frac{\sqrt{N}}{2}, \sqrt{N}]$. Note that there are at most $4 \cdot \sqrt{N}$ light groups. To guarantee full obliviousness, we retrieve a set of size $4 \cdot \sqrt{N}$ that contains all light groups in $x_2$, and each group of size $\sqrt{N}$ contains all light values. 

%Let $x^H_1$ be the set of heavy values returned, with padding up to $\sqrt{N}$ values. %For $i \in \{1,3\}$, we denote the set of tuples whose value in attribute $x_2$ is heavy as $R^H_i$. 
%We compute the following sub-query for outputting all join results whose value in attribute $x_1$ is heavy:
%\begin{align*}
%    \Q^H & = (x^H_1 \times R_2) \ltimes R_1 \ltimes R_3 
%\end{align*}
%More specifically, the Cartesian product of $R_1 \times x^H_2$ is computed by invoking Algorithm~\ref{alg:nestedloop}. Moreover, the result of $R_1 \times x^H_2$ contains all attributes, hence the join with $R_2$ and $R_3$ just degenerates to semi-joins, which can be computed by \semi.

%For light values in $\dom(x_1)$, we further partition them into $\Theta(\sqrt{N})$ groups, such that the total degree of each group falls into $(\frac{\sqrt{n}}{2}, \sqrt{N}]$. For each light group $I$, we first find tuples in $R_1$ and $R_3$, whose values in attribute $x_1$ falls into $I$ and pad up to $\sqrt{N}$ tuples, denoted as $R^I_1, R^I_3$ respectively. We also create dummy light groups and pad up to into $4 \sqrt{N}$ groups. We compute the following sub-query for returning all join results whose value in $x_1$ is light:
%\begin{align*}
%\Q^L & = \bigcup_{I} \left((R^I_1 \Join R^I_3) \ltimes R_2\right) 
%\end{align*}
%More specifically, $R^I_1 \Join R^I_3$ can be simply done by first materializing their Cartesian product $R^I_1 \Join R^I_3$ by invoking Algorithm~\ref{alg:nestedloop}, which incurs a cost of $N$ since $|R^I_1| \le \sqrt{N}$ and $|R^I_3| \le \sqrt{N}$. The semi-join between $R^I_1 \times R^I_3$ and $R_2$ simply degenerates can be computed by the {\sc SemiJoin} primitive.
%
%
%
%\paragraph{Retrieve heavy values.} As described in Algorithm~\ref{alg:heavy} (in Appendix~\ref{appendix:triangle}), $\textsc{ObliviousHeavy}$ takes as input the join query $\Q$, an instance $\R$, an attribute $x$ and a parameter $\tau$, and output every value in attribute $x$ whose degree in $R_e$ is greater than $\frac{|R_e|}{\tau}$ for some relation $e \in \E_x$. This algorithm is built on fully oblivious primitives presented in Section~\ref{sec:preliminary}. More specifically, we first compute the degree of every value in $\dom(x)$ in every relation separately. In a linear scan of (key, degree) pairs obtained, we can replace all light keys with dummy values, and compact the resulted pairs. 
%
%\paragraph{Retrieve Light Groups.} As described in Algorithm~\ref{appendix:triangle} (in Appendix~\ref{appendix:triangle}), $\textsc{ObliviousLight}$ takes as input the join query $\Q$, the instance $\R$, an attribute $x$, and a parameter $\tau$, and attach every tuple with a group id, indicating the light group where it should go into. More specifically, we first compute the degree of every value in $\dom(x)$ in every relation separately. In a linear scan of (key, degree) pairs obtained, we can replace all light keys with dummy values, and compact the resulted pairs. 

%\begin{algorithm}[t]
%\label{alg:heavy}
%\caption{$\textsc{ObliviousHeavy}(\Q = (\V,\E),\R, x, %\tau)$}
%
%$\E_x \gets \{e \in \E: x \in e\}$\;
%\ForEach{$e \in \E_x$}{
%    $S \gets \textsc{CountByKey}(R_e, x)$, $K_e \gets \emptyset$\;
%    \ForEach{$(\key, \cnt) \in S$}{
%        \re $(\key, \cnt)$\;
%        \lIf{$\cnt < \frac{|R_e|}{\tau}$}{\wt $\perp$ to $K_e$}
%        \lElse{\wt $\key$ to $K_e$}
%    }
%    \compact\ $K_e$ and truncate with the first $\tau$ elements\;
%}
%\Return $\bigcup_{e \in \E_x} K_e$\;
%\end{algorithm}

%\begin{algorithm}[t]
%\label{alg:light}
%\caption{$\textsc{ObliviousLight}(\Q = (\V,\E),\R, x, \tau)$}
%
%$\E_x \gets \{e \in \E: x \in e\}$\;
%\ForEach{$e \in \E_x$}{
%    $K_e \gets \textsc{CountByKey}(R_e, x)$\;
%    \ForEach{$(\key, \cnt) \in K_e$}{
%        \lIf{$\cnt > \frac{|R_e|}{\tau}$}{\wt $(\key, 0, e)$}
%        \lElse{\wt $(\key, \cnt, e)$}
%    }
%}
%$K \gets \merge(\bigcup_{e \in \E_x} K_e)$ by $\key$\;
%\lForEach{$e \in \E_x$}{$c_e \gets 0$}
%$\L\gets \emptyset$, $i \gets 0$\;
%\ForEach{$(\key, \{\cnt_e:e \in \E_x\}) \in K$}{
%\If{$c_e + \cnt_e > \frac{|R_e|}{2 \tau}$}{
%    $i \gets i + 1$, \wt $(\key, i)$ to $S$\; 
%    \lForEach{$e \in \E_x$}{$c_e \gets 0$}
%}
%\lElse{\wt $\perp$ to $S$}
%}
%\lForEach{$e \in \E_x$}{$R_e \gets \textsc{MultiSearch}(R_e, x, S)$}
%\Return $\R$\;
%\end{algorithm}



